A Framework to Quantify the Benefits of Network Functions Virtualization in Cellular Networks

Network functions virtualization (NFV) is an appealing vision that promises to dramatically reduce capital and operating expenses for cellular providers. However, existing efforts in this space leave open broad issues about how NFV deployments should be instantiated or how they should be provisioned. In this paper, we present an initial attempt at a framework that will help network operators systematically evaluate the potential benefits that different points in the NFV design space can offer.

==> discussion.tex <==
\section{DISCUSSION}

\begin{itemize}
\item other use cases?
\item other concerns w.r.t isolation etc?
\item how fine-grained are policies in practice?
\end{itemize}

